Bayesian Inference for Regression Copulas

We propose a new semi-parametric distributional regression smoother that is based on a copula decomposition of the joint distribution of the vector of response values. The copula is high-dimensional and constructed by inversion of a pseudo regression, where the conditional mean and variance are semi-parametric functions of covariates modeled using regularized basis functions. By integrating out the basis coefficients, an implicit copula process on the covariate space is obtained, which we call a `regression copula'. We combine this with a non-parametric margin to define a copula model, where the entire distribution - including the mean and variance - of the response is a smooth semi-parametric function of the covariates. The copula is estimated using both Hamiltonian Monte Carlo and variational Bayes; the latter of which is scalable to high dimensions. Using real data examples and a simulation study we illustrate the efficacy of these estimators and the copula model. In a substantive example, we estimate the distribution of half-hourly electricity spot prices as a function of demand and two time covariates using radial bases and horseshoe regularization. The copula model produces distributional estimates that are locally adaptive with respect to the covariates, and predictions that are more accurate than those from benchmark models.

==> acknowl.tex <==

\vspace{0.75em}
\noindent{\large {\bf Acknowledgments}}\\
Nadja Klein gratefully acknowledges funding from the German Alexander von Humboldt foundation. We thank
MutualArt for providing the print price data. 


==> append.tex <==
%\newpage
\appendix
\vspace{-15pt}
\section{}\label{sec:proof}
\vspace{-15pt}
\numberwithin{equation}{section}

\setcounter{equation}{0}
\subsection{Proof of Theorem~\ref{theo:c2}}
\vspace{-10pt}
Recall that $\tilde{\xvec}=\{\xvec,\wvec\}$ and $\thetavec=\{\thetavec_\alpha,\thetavec_\beta\}$, and
note that from Eq.~(\ref{eq:correlationmatrix}) the distribution 
$Z_i|\tilde{\xvec},\thetavec$ is standard normal because
\begin{equation*}\begin{aligned}
p(z_i|\tilde{\xvec},\thetavec)&=\int p_{Z_i}(z_i|\tilde{\xvec},\alphavec,\thetavec_\beta)\,p(\alphavec|\thetavec_{\alpha})\mathrm{d}\alphavec=\int \phi_1(z_i)\,p(\alphavec|\thetavec_{\alpha})\mathrm{d}\alphavec=\phi_1(z_i)\,,
\end{aligned}\end{equation*}
while from Eq.~(\ref{eq:c1}), $p_Z(\zvec|\tilde{\xvec},\alphavec,\thetavec_\beta)=c_1(\uvec|\bm{x},\bm{w},\alphavec,\thetavec_{\beta})\prod_{i=1}^n \phi_1(z_i)$.
Then, the implicit copula density~\cite[Sec 3.1]{Nel2006} of $\bm{Z}|\tilde{\xvec},\thetavec$ is given by
\begin{equation*}\begin{aligned}
c_H(\uvec|\tilde{\xvec},\thetavec)&=\frac{p(\zvec|\tilde{\xvec},\thetavec)}{\prod_{i=1}^n \phi_1(z_i)}=\frac{\int p_Z(\zvec|\tilde{\xvec},\alphavec,\thetavec_\beta)\,p(\alphavec|\thetavec_{\alpha})\mathrm{d}\alphavec}{\prod_{i=1}^n \phi_1(z_i)}\\
&=\frac{\int c_1(\uvec|\bm{x},\bm{w},\alphavec,\thetavec_{\beta})\prod_{i=1}^n \phi_1(z_i) p(\alphavec|\thetavec_{\alpha})\mathrm{d}\alphavec}{\prod_{i=1}^n \phi_1(z_i)}=\int c_1(\uvec|\bm{x},\bm{w},\alphavec,\thetavec_{\beta}) 
p(\alphavec|\thetavec_{\alpha})\mathrm{d}\alphavec\,,
\end{aligned}\end{equation*}
which is the required expression for $c_H$ in Theorem~\ref{theo:c2}. Similarly, if $F_Z(\uvec|\tilde{\xvec},\thetavec)$ denotes
the joint distribution function of $\bm{Z}|\tilde{\xvec},\thetavec$, then its implicit copula function~\citep[Sec.3.1]{Nel2006} is
\begin{eqnarray*}
C_H(\uvec|\tilde{\xvec},\thetavec) &= &F(\zvec|\tilde{\xvec},\thetavec)=\int\int p_Z(\zvec|\tilde{\xvec},\alphavec,\thetavec_\beta)p(\alphavec|\thetavec_\alpha)
\mbox{d}\alphavec \mbox{d}\zvec \\
&= &\int\int \phi(\zvec;\bm{0},R)\mbox{d}\zvec\, p(\alphavec|\thetavec_\alpha) \mbox{d}\alphavec 
= \int \Phi(\zvec;\bm{0},R) p(\alphavec|\thetavec_\alpha) \mbox{d}\alphavec \\
& = &\int C_1(\uvec|\xvec,\wvec,\alphavec,\thetavec_\beta)p(\alphavec|\thetavec_\alpha) \mbox{d}\alphavec\,.
\end{eqnarray*}

\subsection{Proof of Theorem~\ref{theo:Icop}}
First, note that 
$|C_1(\uvec|\xvec,\wvec,\alphavec,\thetavec_\beta)\,p(\alphavec|\thetavec_\alpha)|
\leq M(\uvec)\,p(\alphavec|\thetavec_\alpha)$, where $M(\uvec)$ is the 
upper Fr\'{e}chet-Hoeffding bound. Also note that from 
the definition of $R$ at Eq.~(\ref{eq:correlationmatrix}),
\[
\lim\limits_{ \gamma_\beta \rightarrow 0} R = S^\star \Sigma S^\star= I_n\,,
\]
where $S^\star=\mbox{diag}(\exp(-\vvec_1'\alphavec/2),\ldots,\exp(-\vvec_n'\alphavec/2))$\,.
Then, by Theorem~\ref{theo:c2} and Lebesgue's dominated convergence 
theorem,
\begin{eqnarray*}
	\lim\limits_{ \gamma_\beta \rightarrow 0} C_H(\uvec|\tilde{\xvec},\thetavec) &= &
	\int \lim\limits_{ \gamma_\beta \rightarrow 0} C_1(\uvec|\xvec,\wvec,\thetavec_\beta,\alphavec)\,p(\alphavec|\thetavec_\alpha)\mbox{d}\alphavec\\
	&= &
	\int \lim\limits_{ \gamma_\beta \rightarrow 0} \Phi(\zvec;\bm{0},R)\,p(\alphavec|\thetavec_\alpha)\mbox{d}\alphavec =\int \Phi(\zvec; \bm{0},I)\,p(\alphavec|\thetavec_\alpha)\mbox{d}\alphavec\\
	&= &   \Phi(\zvec; \bm{0},I) =\Phi((\Phi_1^{-1}(u_1),...,\Phi_1^{-1}(u_n))'; 0,I) \\
	&= &\prod_{i=1}^n \Phi_1(\Phi_1^{-1}(u_i))= \Pi(\uvec)\,.
\end{eqnarray*}

\subsection{Derivation of Dependence Metrics in Section~\ref{sec:propertiesC2}}
To derive the lower quantile dependence metric at part~(i), 
\begin{eqnarray*}
	\lambda^L_{ij}(q|\tilde{\xvec},\thetavec)
	&= &\frac{C_H^{ij}(q,q)}{q}= \int \frac{C_1^{ij}(q,q)\,p(\alphavec|\thetavec_\alpha)}{q} \mbox{d}\alphavec=\int \lambda^L_1(q|\xvec,\wvec,\alphavec,\thetavec_\beta)\,p(\alphavec|\thetavec_\alpha) \mbox{d}\alphavec\,.
\end{eqnarray*}
The derivation of the upper quantile dependence is similar.

To derive the metrics at part~(ii), first note that for any bivariate copula function $C$, if $M(u,v)=\max(u,v)$ is the 
upper Fr\'{e}chet-Hoeffding bound, then
$|C(q,q)/q| \leq  M(q,q)/q = 1 $. Denote the $(i,j)$th element of $R$ 
at Eqn.~(\ref{eq:correlationmatrix}) as $r_{ij}$, and the sub-copulas
of $C_1$ and $C_H$ in these elements as $C_1^{ij}$ and $C_H^{ij}$. 
Then, by Theorem~\ref{theo:c2} and Lebesgue's dominated convergence 
theorem,
\[
\lambda^L_{ij}  = \lim\limits_{q \downarrow 0} \frac{C_H^{ij}(q,q)}{q}
=  \int\lim\limits_{q \downarrow 0}\frac{C_1^{ij}(q,q)}{q} p(\alphavec|\thetavec_\alpha) \mbox{d}\alphavec = 0
\]
because $C_1^{ij}$ is a Gaussian copula with zero tail dependence, so that
$\lim\limits_{q \downarrow 0}\frac{C_1^{ij}(q,q)}{q}=0$. 
The derivation of $\lambda^U$ is similar.

The derivation of $\rho^S_{ij}$ in part~(iii) follows from the definition
of Spearman's correlation, and its expression for a Gaussian copula, as follows:
\begin{eqnarray*}
\rho^S_{ij}(\tilde{\xvec},\thetavec)
 &= &12 \int C_H^{ij}(u,v)\mbox{d}(u,v)-3 = 12 \int \int C_1^{ij}(u,v)\,p(\alphavec|\thetavec_\alpha)\mbox{d}(u,v)\mbox{d}\alphavec -3\\
 &= & \int \left( 12\int C_1^{ij}(u,v)\mbox{d}(u,v)-3+3\right)\,p(\alphavec|\thetavec_\alpha) \mbox{d}\alphavec -3\\
 &= &\frac{6}{\pi} \int \arcsin(r_{ij}/2)\,p(\alphavec|\thetavec_{\alpha})\mbox{d}\alphavec\,.
\end{eqnarray*}
The derivation of $\tau^K_{ij}$ in part~(iv) is similar. 

%\subsection{Proof of Theorem~\ref{theo:volatility}}\label{sec:proof:theo:vol}
%\vspace{-10pt}
%\begin{proof}
%First, the $\mathcal{C}^0$  function $V(\cdot)$, $V:\dsR^+\to\dsR^+$ has the property that $V^-(V(y_j-\mu_Y))=|y_j-\mu_Y|$ such that the values $v_j$ can be mapped to $y_j$ in a one-to-two transformation via $y_j=(-1)^l V^-(v_j)+\mu_Y$, for $l\in\lbrace 1,2\brace$.
%Since $V^{-}V(y_j-\mu_Y)$ is deterministic, the joint distribution of $(V_1,V_2)$ is given by
%\begin{equation*}\begin{aligned}
%F_V(v_1,v_2)&=\dsP(-V^{-}(v_1)\leq Y_1-\mu_Y\leq V^{-}(v_1),-V^{-}(v_2)\leq Y_2-\mu_Y\leq V^{-}(v_2))\\
%&\quad=\sum_{j,k=1}^2(-1)^j(-1)^k F((-1)^jV^-(v_1)+\mu_Y,(-1)^jV^-(v_2)+\mu_Y).
%\end{aligned}\end{equation*}
%By Sklar's Theorem we furthermore know that the joint distribution of $Y$ can be written as $F(y_1,y_2)=C(F_Y(y_1),F_Y(y_2))$ such that
%\begin{equation*}\begin{aligned}
%F_V(v_1,v_2)&=\sum_{j,k=1}^2(-1)^j(-1)^k C(F_Y((-1)^jV^-(v_1)+\mu_Y),F_Y((-1)^jV^-(v_2)+\mu_Y)).
%\end{aligned}\end{equation*}
%Inverting Sklar's Theorem for $  u_j=F_V(v_j)$ and marginal distributions $F_V$ of $V_j$ we finally obtain
%\begin{equation*}\begin{aligned}
%C_V(  u_1,  u_2)&=F_V(F_V^{-1}(v_1),F_V^{-1}(v_2))\\
%&=\sum_{j,k=1}^2(-1)^j(-1)^k {C}(F_Y(\mu_Y+(-1)^jV^-(F_V^{-1}(  u_1)),F_Y(\mu_Y+(-1)^kV^-(F_V^{-1}(  u_2))),
%\end{aligned}\end{equation*}
%and where 
%\begin{equation*}\begin{aligned}
%F_V(v_j)&=\dsP(V_j\leq v_j)=\dsP(-V^-(v_j)\leq Y_1-\mu_Y\leq V^-(v_j))\\
%&=F_Y(V^{-}(v_j)+\mu_Y)-F_Y(-V^{-}(v_j)+\mu_Y).
%\end{aligned}\end{equation*}
%The copula density in Eq~\eqref{cond:var:cop:dens} follows from differentiating Eq~\eqref{cond:var:cop}.
%\begin{equation*}\begin{aligned}
%c_V(  u_1,  u_2)&=\frac{\partial^2}{\partial u_1\partial u_2}C_V(u_1,u_2)
%\frac{\tfrac{\partial}{\partial v_1}V^{-}(F_V^{-1}(  u_1))\frac{\partial}{\partial v_2}V^{-}(F_V^{-1}(  u_2))}{p_V(F_V^{-1}(  u_1))p_V(F_V^{-1}(  u_2))}\\&\quad\times\sum_{j,k=1}^2(-1)^j(-1)^k {c}(F_V(\mu_Y+(-1)^jV^-(F_V^{-1}(  u_1)),F_V(\mu_Y+(-1)^kV^-(F_V^{-1}(  u_2)))\\
%&=\frac{\tfrac{\partial}{\partial v_1}V^{-}(F_V^{-1}(  u_1))\frac{\partial}{\partial v_2}V^{-}(F_V^{-1}(  u_2))}{p_V(F_V^{-1}(  u_1))p_V(F_V^{-1}(  u_2))}\\&\quad\times\sum_{j,k=1}^2(-1)^j(-1)^k {p}(F_V(\mu_Y+(-1)^jV^-(F_V^{-1}(  u_1)),F_V(\mu_Y+(-1)^kV^-(F_V^{-1}(  u_2))),
%\end{aligned}\end{equation*}
%where $p$ denotes the joint density of of $Y$.
%\end{proof}

%\vspace{-15pt}
%\section{Details on Posterior Estimation}\label{app:sec:derivs:iwls}
%\vspace{-10pt}
%In this appendix we provide the derivatives and computational details required 
%for the efficient implementation
%of the HetPSC with exact method and VB in Section~\ref{subsec:est}.
%
%\vspace{-12pt}
%\subsection{Exact Inference}\label{app:subsec:derivatives}
%\vspace{-7pt}
%
%
%\subsubsection{Derivatives of $\thetavec_{\beta}$}\label{blubb}
%We update $\tau^2_{\beta},\psi_{\beta,1},\psi_{\beta,2}$ separately. First and second derivatives of~\eqref{eq:logFC:xi} with respect to $\tilde\psi_{\beta,j}$ are
%\begin{equation}\label{eq:tau2:beta}
%\begin{aligned}
%\frac{\partial l_{\tilde\psi_{\beta,j}^2}}{\partial\tilde\psi_{\beta,j} }&=   \frac{\partial}{\partial{\tilde\psi_{\beta,j}}} \log\left(\frac{\partial{\psi_{\beta,j}}}{\partial{\tilde\psi_{\beta,j}}}\right) - \frac{1}{2} \sum_{i=1}^{n} \frac{\partial}{\partial{\tilde\psi_{\beta,j}}}s_{i}^{2} + \frac{1}{2} \frac{\partial}{\partial{\tilde\psi_{\beta,j}}} (SS')^{-1} + \betavec'B'\frac{\partial}{\partial{\tilde\psi_{\beta,j}}}S^{-1}\zvec \\
%&\quad - \frac{1}{2} \betavec'\frac{\partial}{\partial{\tilde\psi_{\beta,j}}}P(\thetavec_{\beta})(\tilde\psi_{\beta,j})\betavec + \frac{1}{2} \frac{\partial}{\partial{\tilde\psi_{\beta,j}}} \log(\det(\Delta_{\beta}))\\
%\frac{\partial^2 l_{\tilde\psi_{\beta,j}^2}}{\partial\tilde\psi_{\beta,j}^2 }&=  \frac{\partial^2}{\partial{\tilde\psi_{\beta,j}^2}} \log\left(\frac{\partial{\psi_{\beta,j}}}{\partial{\tilde\psi_{\beta,j}}}\right) - \frac{1}{2} \sum_{i=1}^{n} \frac{\partial^2}{\partial{\tilde\psi_{\beta,j}^2}}s_{i}^{2} + \frac{1}{2} \frac{\partial^2}{\partial{\tilde\psi_{\beta,j}^2}} (SS')^{-1} + \betavec'B'\frac{\partial^2}{\partial{\tilde\psi_{\beta,j}^2}}S^{-1}\zvec \\
%&\quad - \frac{1}{2} \betavec'\frac{\partial^2}{\partial{\tilde\psi_{\beta,j}^2}}P(\thetavec_{\beta})\betavec + \frac{1}{2} \frac{\partial^2}{\partial{\tilde\psi_{\beta,j}^2}} \log(\det(\Delta_{\beta})), \\
%\end{aligned}
%\end{equation}
%for which we computed the following derivatives:
%% Let $\gamma_{\beta,0}=\frac{\tau_{\beta}^2}{(1-\tilde\psi_{\beta,1}^{2})(1-\tilde\psi_{\beta,2}^{2})}$ and $\tilde P_{\beta}$ such that $\gamma_{\beta,0} (1-\tilde\psi_{\beta,1}^{2})(1-\tilde\psi_{\beta,2}^{2})\tilde P_{\beta}^{-1}=P(\thetavec_{\beta})^{-1}$. Then,
%\begin{equation*}
%\begin{aligned}
%%s_{i}^{2} &= \left(1 + \gamma_{\beta,0} (1-\tilde\psi_{\beta,1}^{2})(1-\tilde\psi_{\beta,2}^{2})\bvec_{i}'\tilde P_{\beta}^{-1}\bvec_{i}\right)^{-1} \mbox{ and hence }\\
%\frac{\partial{s_{i}^{2}}}{\partial{\tilde\psi_{\beta,j}}} &= - (s_{i}^{2})^{2} \frac{\partial}{\partial{\tilde\psi_{\beta,j}}} \bvec_{i}'P(\thetavec_{\beta})^{-1}\bvec_{i} \\
%%&= - \frac{\gamma_{0} (1-\tilde\psi_{\beta,2}^{2})}{(s_{i}^{2})^{2}} \left[-2\tilde\psi_{\beta,1} \bvec_{i}'\tilde P_{\beta}^{-1}\bvec_{i} + (1-\tilde\psi_{\beta,1}^{2}) \frac{\partial}{\partial{\tilde\psi_{\beta,1}}} \bvec_{i}'\tilde P_{\beta}^{-1}\bvec_{i}\right] \\
%\frac{\partial^2{s_{i}^{2}}}{\partial{\tilde\psi_{\beta,j}^{2}}} &= 2(s_{i}^{2})^{3}\frac{\partial{s_{i}^{2}}}{\partial{\tilde\psi_{\beta,j}}}  \frac{\partial}{\partial{\tilde\psi_{\beta,1}}}\bvec_{i}'P(\thetavec_{\beta})^{-1}\bvec_{i}   - (s_{i}^{2})^{2} \frac{\partial^2}{\partial{\tilde\psi_{\beta,j}}^2}\bvec_{i}'P(\thetavec_{\beta})^{-1}\bvec_{i},
%\end{aligned} 
%\end{equation*}
%and where
%\begin{equation*}
%\begin{aligned}
%(\Delta_{\beta})_{ij}&=\begin{cases}1 & \mbox{if } i=j\mbox{ and } i\neq 1,2\\
%-\psi_{\beta,2} & \mbox{if } i=j+2 \\
%-\psi_{\beta,1}(1-\psi_{\beta,2}) & \mbox{if } i=j+1\mbox{ and } i\neq 1,2\\
%\sqrt{1-\psi_{\beta,1}^2}\sqrt{1-\psi_{\beta,2}^2} & \mbox{if } i=j=1\\
%(1-\psi_{\beta,2}^2) & \mbox{if } i=j=2\\
%-\psi_{\beta,1}\sqrt{1-\psi_{\beta,2}^2} & \mbox{if } i=2\mbox{ and } j=1.\end{cases}
%\end{aligned}
%\end{equation*}
%Then, we use that $\frac{\partial}{\partial{\tilde\psi_{\beta,j}}}(\Delta_{\beta})_{ij}=\frac{\partial\psi_{\beta,j}}{\partial{\tilde\psi_{\beta,j}}}\frac{\partial}{\partial{\psi_{\beta,j}}}(\Delta_{\beta})_{ij}$, with
%\begin{equation*}
%\begin{aligned}
%\frac{\partial\psi_{\beta,j}}{\partial{\tilde\psi_{\beta,j}}}&=\frac{2\exp(\tilde\psi_{\beta,j})(1-\epsilon)}{(1+\exp(\tilde\psi_{\beta,j}))^2}\\
%\frac{\partial}{\partial{\tilde\psi_{\beta,j}}}\log\left(\frac{\partial\psi_{\beta,j}}{\partial{\tilde\psi_{\beta,j}}}\right)&=1-\frac{2\exp(\tilde\psi_{\beta,j})}{1+\exp(\tilde\psi_{\beta,j})}.
%\end{aligned}
%\end{equation*}
%Then, 
%\begin{equation*}
%\begin{aligned}
%\frac{\partial}{\partial{\psi_{\beta,j}}}P(\psivec_{\beta}) &= \left(\frac{\partial}{\partial{\psi_{\beta,j}}}\Delta_{\beta}'\right)\Delta_{\beta}  + \Delta_{\beta}' \frac{\partial}{\partial{\psi_{\beta,j}}}\Delta_{\beta} \\
%\frac{\partial}{\partial{\psi_{\beta,1}}}\delta_{11} 
%&= - \frac{\psi_{\beta,1}^{2} \sqrt{(1-\psi_{\beta,2}^{2})}}{\sqrt{1-\psi_{\beta,1}^{2}}} \\
%\frac{\partial}{\partial{\psi_{\beta,2}}}\delta_{11} &=  - \frac{\psi_{\beta,2}^{2} \sqrt{1-\psi_{\beta,1}^{2}}}{\sqrt{1-\psi_{\beta,2}^{2}}} \\
%\frac{\partial}{\partial{\psi_{\beta,1}}}\delta_{21} &=- \sqrt{1-\psi_{\beta,2}^{2}} \hspace{1cm} \frac{\partial}{\partial{\psi_{\beta,2}}}\delta_{21} = \frac{\psi_{\beta,1}\psi_{\beta,2}}{\sqrt{1-\psi_{\beta,2}^{2}}}\\
%\frac{\partial}{\partial{\psi_{\beta,1}}}\delta_{22} &= 0 \hspace{2.95cm} \frac{\partial}{\partial{\psi_{\beta,2}}}\delta_{22} =  - \frac{\psi_{\beta,2}}{\sqrt{1-\psi_{\beta,2}^{2}}} \\
%\frac{\partial}{\partial{\psi_{\beta,1}}}\delta_{31} &= 0 \hspace{2.95cm} \frac{\partial}{\partial{\psi_{\beta,2}}}\delta_{31} = -1 \\
%\frac{\partial}{\partial{\psi_{\beta,1}}}\delta_{32} &= -(1-\psi_{\beta,2}) \hspace{1.1cm} \frac{\partial}{\partial{\psi_{\beta,2}}}\delta_{32} = \psi_{\beta,1}, 
%\end{aligned}
%\end{equation*}
%\begin{equation*}
%\begin{aligned}
%\frac{\partial}{\partial{\psi_{\beta,1}}}\log(\det(P)^{\frac{1}{2}}) &= -\frac{1}{1-\psi_{\beta,1}^{2}}  \\\frac{\partial}{\partial{\psi_{\beta,2}}}\log(\det(P)^{\frac{1}{2}})&=- \frac{2\psi_{\beta,2}^{2}}{(1-\psi_{\beta,2}^{2})^{2}}.
%\end{aligned}
%\end{equation*}
%
%
%
%
%\subsubsection{Gradient of $\alphavec$}
%\begin{equation}\label{eq:grad:alpha}
%\begin{aligned}
%&\nabla_{\alpha} l_{\alpha}=-\frac{1}{2}P(\thetavec_{\alpha})\alphavec\\ &+V'\left\lbrack\left(\frac{\partial s_1^2}{\partial\alphavec}s_1^{-2},\ldots,\frac{\partial s_n^2}{\partial\alphavec}s_n^{-2}\right)+\left(\frac{\partial s_1^2}{2\partial\alphavec}z_1^2 s_1^{-4},\ldots,\frac{\partial s_n^2}{2\partial\alphavec}z_n^2 s_n^{-4}\right)+\frac{1}{2}\zvec'\circ\left( \frac{\partial s_1^2}{\partial\alphavec}s_1^{-3},\ldots,\frac{\partial s_n^2}{\partial\alphavec}s_n^{-2}\right)\circ (\beta'B')         \right\rbrack
%\end{aligned}
%\end{equation}
%
%\subsubsection{Derivatives of $\thetavec_{\alpha}$}
%We update $\tau^2_{\alpha},\psi_{\alpha,1},\psi_{\alpha,2}$ separately. First and second derivatives of~\eqref{eq:logFC:tau2:alpha} with respect to $\tilde\tau^2_{\alpha}$ are
%\begin{equation*}\label{eq:tau2:alpha}
%\begin{aligned}
%\frac{\partial l_{\tilde\tau_{\alpha}^2}}{\partial\tilde\tau_{\alpha}^2 }&=    -\frac{1}{2}(p_{\alpha}-1) - \frac{1}{2} \left(\frac{\exp(\tilde\tau_{\alpha}^2)}{b_{0}}\right)^{\frac{1}{2}} + \frac{1}{2 \exp(\nu)} \alphavec'P(\thetavec_{\alpha})\alphavec \\
%\frac{\partial^2 l_{\tilde\tau_{\alpha}^2}}{\partial(\tilde\tau_{\alpha}^2)^2 }&=    -\frac{1}{4}\left(\frac{\exp(\tilde\tau_{\alpha}^2)}{b_{0}}\right)^{\frac{1}{2}} - \frac{1}{2\exp(\tilde\tau_{\alpha}^2)} \alphavec'P(\thetavec_{\alpha})\alphavec\\
%\end{aligned}
%\end{equation*}
%Furthermore, derivatives of~\eqref{eq:logFC:psi:alpha} with respect to $\tilde\psi_{\alpha,1}$ are
%\begin{equation*}
%\begin{aligned}
%\frac{\partial{l_{\tilde\psi_{\alpha,j}}}}{\partial{\tilde\psi_{\alpha,j}}} &\propto \frac{\partial}{\partial{\tilde\psi_{\alpha,j}}} \log(\det(\Delta_{\alpha})) - \alphavec' \frac{1}{2\tau_{\alpha}^{2}} \frac{\partial}{\partial{\tilde\psi_{\alpha,j}}}P(\tilde\psi_{\alpha,j})\alphavec + \frac{\partial}{\partial{\tilde\psi_{\alpha,j}}}\left(\log\left(\frac{\partial{\psi_{\alpha,j}}}{\partial{\tilde\psi_{\alpha,j}}}\right)\right) \\
%\frac{\partial^2{l_{\tilde\psi_{\alpha,j}}}}{\partial{\tilde\psi_{\alpha,j}^2}} &\propto \frac{\partial^2}{\partial{\tilde\psi_{\alpha,j}^2}} \log(\det(\Delta_{\alpha})) - \alphavec' \frac{1}{2\tau_{\alpha}^{2}} \frac{\partial^2}{\partial{\tilde\psi_{\alpha,j}^2}}P(\tilde\psi_{\alpha,j})\alphavec + \frac{\partial^2}{\partial{\tilde\psi_{\alpha,j}^2}}\left(\log\left(\frac{\partial{\psi_{\alpha,j}}}{\partial{\tilde\psi_{\alpha,j}}}\right)\right), \\
%\end{aligned}
%\end{equation*}
%and where the derivatives of $\log(\det(\Delta_{\alpha}))$ and $P(\thetavec_{\alpha})$ with respect to $\tilde\psi_{\alpha,j}$ follow the formulas given before.
%
%\vspace{-12pt}
%\subsection{Variational Inference}\label{app:subsec:vb}
%\vspace{-7pt}
%
%For VB, the Hessians are not required. Gradients of $\tilde\psi_{\beta,j}$, $\alphavec$ and $\thetavec_{\alpha}$ are given in the previous subsection. The one of $\tilde\tau_{\beta,j}^2$ is straightforward with the Appendix of~\citet{KleSmi2017}. The one of the conditional posterior of $\betavec$ $l_{\beta}$ is \textbf{MIKE please check as well.}
%\[
%\nabla_{\beta}l_{\beta}=B'S^{-1}\zvec-(B'B+P(\thetavec_{\beta}))\betavec.
%\]





==> figs_WA.tex <==
\begin{figure}[t]
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_rents.eps}}\\%\hspace{0.3cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_nigeria.eps}}\\
%\hspace{0.6cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_amazon.eps}}\\%\vspace{0.2cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_incomes.eps}}\\
%\centering{\includegraphics[width=0.975\textwidth,angle=0]{Figures/dep_amazon.eps}}\hspace{0.3cm}
%\centering{\includegraphics[width=0.975\textwidth,angle=0]{Figures/dep_incomes.eps}}
\caption{Upper quantile dependence $\lambda^U(0.99)$. The datasets are (a,b) \texttt{Rents}, (c,d) \texttt{Nigeria}, (e,f) \texttt{Amazon},
and (g,h) \texttt{Incomes}.}\label{fig:dep:qu}
\end{figure}


\begin{figure}[t]
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_geyser_tauk_R1.eps}}\\%\hspace{0.3cm}

\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_rents_tauk.eps}}\\%\hspace{0.3cm}
%\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_nigeria_tauk.eps}}\\
%\hspace{0.6cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_amazon_tauk.eps}}\\%\vspace{0.2cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_incomes_tauk.eps}}\\
%\centering{\includegraphics[width=0.975\textwidth,angle=0]{Figures/dep_amazon.eps}}\hspace{0.3cm}
%\centering{\includegraphics[width=0.975\textwidth,angle=0]{Figures/dep_incomes.eps}}
\caption{Kendall's tau $\tau^k$. The datasets are (a,b) \texttt{Geyser}, (c,d) \texttt{Rents}, (e,f) \texttt{Amazon},
and (g,h) \texttt{Incomes}.}\label{fig:dep:kendall}
\end{figure}



\begin{figure}[t]
{\includegraphics[width=0.99\textwidth,angle=0]{Figures/params_sd_R1_new.eps}}%\hspace{1cm}
\caption{Standard deviation estimates of $\betavec$ (blue) and $\alphavec$ (if $\neq\nullvec$) of VB against HMC/MCMC. The datasets are (a,b) \texttt{Geyser}, (c,d) \texttt{Rents}, (e,f) \texttt{Amazon},
and (g,h) \texttt{Incomes}. HPSC is shown in panels (a,c,e,g) and PSC in (b,d,f,h).}\label{fig:params}
\end{figure}


\begin{figure}[t]
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_geyser_spearvar_R1.eps}}\\
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_rents_spearvar.eps}}\\%\hspace{0.3cm}
%\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_nigeria_spearvar.eps}}\\
%\hspace{0.6cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_amazon_spearvar.eps}}\\%\vspace{0.2cm}
\centering{\includegraphics[width=0.825\textwidth,angle=0]{Figures/dep_incomes_spearvar.eps}}\\
%\centering{\includegraphics[width=0.975\textwidth,angle=0]{Figures/dep_amazon.eps}}\hspace{0.3cm}
%\centering{\includegraphics[width=0.975\textwidth,angle=0]{Figures/dep_incomes.eps}}
\caption{Spearman's rho $\rho_V^s$ of $C_V$. The datasets are (a,b) {\tt Geyser}, (c,d) {\tt Rents}, (e,f) {\tt Amazon}, and (g,h) {\tt Incomes}.}\label{fig:vdep:spear}
\end{figure}

\begin{figure}[t]
\centering{\includegraphics[width=0.5\textwidth,angle=0]{Figures/LB_amazon_add.eps}}%\hspace{1cm}
\caption{Variational lower bound ${\cal L}(\bm{\lambda})$ with $K=20$ factors for the Amazon data in the additive model with HPSC and VB.}\label{fig:amazon:LB_add}
\end{figure}

\begin{figure}[t]
{\includegraphics[width=0.99\textwidth,angle=0]{Figures/predy_amazon_add.eps}}%\hspace{1cm}
\caption{Posterior estimates of the regression functions $m(x_0,x_0)$ (left-hand side) and 
		variance functions $v(x_0,x_0)$ (right-hand side) on a dense bivariate grid of $(x_0,x0)$ for the Amazon data in the additive model with HPSC and VB.}\label{fig:amazon:predy_add}
\end{figure}
